One-Shot Learning on Attributed Sequences

One-shot learning has become an important research topic in the last decade with many real-world applications. The goal of one-shot learning is to classify unlabeled instances when there is only one labeled example per class. Conventional problem setting of one-shot learning mainly focuses on the data that is already in feature space (such as images). However, the data instances in real-world applications are often more complex and feature vectors may not be available. In this paper, we study the problem of one-shot learning on attributed sequences, where each instance is composed of a set of attributes (e.g., user profile) and a sequence of categorical items (e.g., clickstream). This problem is important for a variety of real-world applications ranging from fraud prevention to network intrusion detection. This problem is more challenging than conventional one-shot learning since there are dependencies between attributes and sequences. We design a deep learning framework OLAS to tackle this problem. The proposed OLAS utilizes a twin network to generalize the features from pairwise attributed sequence examples. Empirical results on real-world datasets demonstrate the proposed OLAS can outperform the state-of-the-art methods under a rich variety of parameter settings.

==> envdef.tex <==
%% --- Definition and Newcommand Zone ---
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}
%\newcommand*{\affmark}[1][\dag]{\textsuperscript{#1}}
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}

\newcommand{\sysname}{\textsf{OLAS} }
\newcommand{\sysnamens}{\textsf{OLAS}}
%\newcommand{\attnet}{\texttt{Attribute Network} }
% \newcommand{\anet}{\texttt{AttNet} }
% \newcommand{\anetns}{\texttt{AttNet}}
% %\newcommand{\seqnet}{\texttt{Sequence Network} }
% \newcommand{\snet}{\texttt{SeqNet} }
% \newcommand{\snetns}{\texttt{SeqNet}}
\newcommand{\vnet}{\textsf{PredictNet} }
\newcommand{\vnetns}{\textsf{PredictNet}}
%\newcommand{\fusenet}{\texttt{Fusion Network} }
\newcommand{\cnet}{\textsf{CoreNet} }
\newcommand{\cnetns}{\textsf{CoreNet}}
\newcommand{\rulesep}{\unskip\ \vrule\ }
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\etc}{\emph{etc}}
\newtheorem{motivation}{Motivating Example}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.8}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\newcommand\smallcaption[1]{%
  \captionsetup{font=normal}%
  \caption{#1}}
  
\usepackage{varwidth}
\DeclareCaptionFormat{centercaption}{%
  % #1: label (e.g. "Table 1")
  % #2: separator (e.g. ": ")
  % #3: caption text
  \begin{varwidth}{\linewidth}%
    \centering
    #1#2#3%
  \end{varwidth}%
}
  
\clubpenalty=10000 
\widowpenalty = 10000
\DeclareMathOperator{\var}{var}
\renewcommand{\vec}[1]{\bm{#1}}
\algnewcommand\algorithmicinput{\textbf{INPUT:}}
\algnewcommand\INPUT{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{OUTPUT:}}
\algnewcommand\OUTPUT{\item[\algorithmicoutput]}
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
%% --- End of Definition and Newcommand Zone ---

==> templates/acm/envdef.tex <==
%% --- Definition and Newcommand Zone ---

\newcommand{\sysname}{\texttt{OLAS} }
\newcommand{\sysnamens}{\texttt{OLAS}}
%\newcommand{\attnet}{\texttt{Attribute Network} }
\newcommand{\anet}{\texttt{A-Net} }
\newcommand{\anetns}{\texttt{A-Net}}
%\newcommand{\seqnet}{\texttt{Sequence Network} }
\newcommand{\snet}{\texttt{S-Net} }
\newcommand{\snetns}{\texttt{S-Net}}
\newcommand{\vnet}{\texttt{PredictNet} }
\newcommand{\vnetns}{\texttt{PredictNet}}
%\newcommand{\fusenet}{\texttt{Fusion Network} }
\newcommand{\fnet}{\texttt{ASN} }
\newcommand{\fnetns}{\texttt{ASN}}
% \newcommand{\mnet}{\texttt{MetricNet} }
% \newcommand{\mnetns}{\texttt{MetricNet}}
\newcommand{\rulesep}{\unskip\ \vrule\ }
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\etc}{\emph{etc}}
\newtheorem{example}{Motivating Example}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmin}{arg\,min}

\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.8}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\newcommand\smallcaption[1]{%
  \captionsetup{font=normal}%
  \caption{#1}}
  
\usepackage{varwidth}
\DeclareCaptionFormat{centercaption}{%
  % #1: label (e.g. "Table 1")
  % #2: separator (e.g. ": ")
  % #3: caption text
  \begin{varwidth}{\linewidth}%
    \centering
    #1#2#3%
  \end{varwidth}%
}
  
\clubpenalty=10000 
\widowpenalty = 10000
\DeclareMathOperator{\var}{var}
\renewcommand{\vec}[1]{\bm{#1}}
\algnewcommand\algorithmicinput{\textbf{INPUT:}}
\algnewcommand\INPUT{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{OUTPUT:}}
\algnewcommand\OUTPUT{\item[\algorithmicoutput]}
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
%% --- End of Definition and Newcommand Zone ---

==> templates/springer/envdef.tex <==
%% --- Definition and Newcommand Zone ---
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}
%\newcommand*{\affmark}[1][\dag]{\textsuperscript{#1}}
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}

\newcommand{\sysname}{\textsc{Olas} }
\newcommand{\sysnamens}{\textsc{Olas}}
%\newcommand{\attnet}{\texttt{Attribute Network} }
% \newcommand{\anet}{\texttt{AttNet} }
% \newcommand{\anetns}{\texttt{AttNet}}
% %\newcommand{\seqnet}{\texttt{Sequence Network} }
% \newcommand{\snet}{\texttt{SeqNet} }
% \newcommand{\snetns}{\texttt{SeqNet}}
\newcommand{\vnet}{\textsc{PredictNet} }
\newcommand{\vnetns}{\textsc{PredictNet}}
%\newcommand{\fusenet}{\texttt{Fusion Network} }
\newcommand{\cnet}{\textsc{CoreNet} }
\newcommand{\cnetns}{\textsc{CoreNet}}
\newcommand{\rulesep}{\unskip\ \vrule\ }
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\etc}{\emph{etc}}
\newtheorem{motivation}{Motivating Example}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.8}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\newcommand\smallcaption[1]{%
  \captionsetup{font=normal}%
  \caption{#1}}
  
\usepackage{varwidth}
\DeclareCaptionFormat{centercaption}{%
  % #1: label (e.g. "Table 1")
  % #2: separator (e.g. ": ")
  % #3: caption text
  \begin{varwidth}{\linewidth}%
    \centering
    #1#2#3%
  \end{varwidth}%
}
  
\clubpenalty=10000 
\widowpenalty = 10000
\DeclareMathOperator{\var}{var}
\renewcommand{\vec}[1]{\bm{#1}}
\algnewcommand\algorithmicinput{\textbf{INPUT:}}
\algnewcommand\INPUT{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{OUTPUT:}}
\algnewcommand\OUTPUT{\item[\algorithmicoutput]}
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
%% --- End of Definition and Newcommand Zone ---
